Chiral-odd gluon generalized parton distributions in the proton: A light-front quantization approach

Within the basis light-front quantization (BLFQ) framework, we evaluate the gluon chiral-odd generalized parton distributions (GPDs) inside the proton at zero skewness. We employ the light-front wave functions of the proton obtained from a light-front quantized Hamiltonian with quantum chromodynamics input using BLFQ. Our investigation encompasses both the valence Fock sector with three constituent quarks and an additional sector containing three quarks and a dynamical gluon. We analyze the gluon GPDs in the momentum space as well as in the transverse position space. We further present the gluon's generalized form factors derived from the Mellin moments of its chiral-odd GPDs. Using the proton transverse spin sum rule, we also present the $x$-dependence of the angular momentum carried by the polarized gluon and determine the relative contributions of quarks and the gluon to the transversity asymmetry.

==> preamble_math_physics.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 1.math mode general functionalities %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%载入必要包
\usepackage{amsmath,amssymb,mathtools} %这行代码载入了三个包：
%amsmath： 提供各种数学环境和符号，用于排版公式和方程。
%amssymb： 提供额外的数学符号，包括双线字体字母 (mathbb)、希腊字母等等。
%mathtools： 在 amsmath 的基础上，提供额外功能用于排版复杂的公式和定理。

\ifpdftex
  \ifxetex
    \usepackage{xcolor}
  \else
    \usepackage{color}
  \fi
\else
  \usepackage{color}
\fi

\ifpdftex%\ifpdftex ... \else ... \fi： 这个条件语句根据编译器是否为 PDFTeX 来设置不同的字体配置。
	% \usepackage[notext]{stix2} %是一个 LaTeX 包的调用，用于加载 STIX2 字体系列。该包提供了多种数学和科学符号，以及一些额外的字体，例如用于数学公式的字体和用于文本的字体。如果您只需要使用 STIX2 中的少数符号，可以使用\usepackage{amsmath} 和 \usepackage{amssymb} 等其他包来代替。
	\usepackage{bbm}
	\newcommand{\mybb}[1]{\mathbbm{#1}}
	\newcommand{\mybf}[1]{\boldsymbol{#1}}
	\newcommand{\mycal}[1]{\mathcal{#1}}
\else
	\usepackage[bold-style=ISO]{unicode-math} %载入 unicode-math 包，提供高级字体处理和更广泛的数学字体。
    %CCC unicode-math for a better scheme to change the math font and also to render different style like \symbf \symbb \symit et al. But, if one only need to get an italic boldface then one could simply use \usepackage{bm}, \pmb{p}, \boldsymbol{p}. If one just want to extend the original \mathbb command to, for example, correctly showing blackboard style number, one may just use \usepackage{bbm}, \usepackage{stix2}. A list of useable math font can be found on: https://tug.org/pracjourn/2006-1/hartke/hartke.pdf and https://tex.stackexchange.com/a/30066/239820
	\setmathfont{latinmodern-math.otf} %设置主数学字体为 Latin Modern Math.
	\setmathfont[range=bb]{TeX Gyre DejaVu Math} %设置黑板粗体字体为 TeX Gyre DejaVu Math.
	\newcommand{\mybb}[1]{\symbb{#1}} %使用 unicode-math 中的 \symbb 定义 \mybb 来表示黑板粗体。
	\newcommand{\mybf}[1]{\symbf{#1}} %使用 \symbf 定义 \mybf 在数学模式中加粗文本。
	\newcommand{\mycal}[1]{\symcal{#1}} %使用 \symcal 定义 \mycal 来表示花体字母。
\fi


\usepackage{siunitx}  
%这行代码加载了 siunitx 宏包，这是一个用于在 LaTeX 文档中排版物理量和单位的强大工具。它提供了：
%单位的一致格式化，包括适当的间距和字体。
%自动处理单位转换和计算。
%对各种单位系统（SI、美国习惯单位等）的支持。
%CCC basically provide those three powerful macro \num, \ang, \si to express physical number with unit properly.
	\sisetup{detect-all = true}
%这行代码配置 siunitx 宏包以自动检测和格式化文本中的物理量。这意味着：
%当您键入一个数字值后跟单位符号（例如 10 cm、2.5 kg、300 K）时，siunitx 会自动识别它为物理量并进行相应的格式化。
%您不需要为每个量显式使用 \SI 或 \num 等命令。

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 2.math-related %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 2.a.general purpose %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    %CCC to produce delimiter of arbitrary size. usage: \vast{2}|
\makeatletter
\newcommand{\vast}[1]{\bBigg@{#1}}
\makeatother
    
\newcommand{\abs}[1]{\left|#1\right|}

\newcommand{\queseq}{\pmb{\quesclr \stackrel{\mbox{?}}{=}\color{black}}}
\newcommand{\intd}[3][]{\ifthenelse{\isempty{#3}}{\mathrm{d}^{#1} #2}{\frac{\mathrm{d}^{#1} #2}{#3}}\;}
\newcommand{\rmd}{\mathrm{d}}


    %CCC long equal sign with text above it. the equal sign will not extend according to the length of the text
\newcommand{\eqtext}[1]{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\small\rmfamily #1}}}{=}}}
\newcommand{\Leqtext}[1]{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\small\rmfamily #1}}}{=\mathrel{\mkern-3mu}=}}}
\newcommand{\LLeqtext}[1]{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\small\rmfamily #1}}}{=\mathrel{\mkern-3mu}=\mathrel{\mkern-3mu}=}}}
\usepackage{stackengine}
\newcommand{\stackequal}[2]{%
    \mathrel{\stackunder[2pt]{\stackon[4pt]{=\mathrel{\mkern-3mu}=\mathrel{\mkern-3mu}=}{$\scriptscriptstyle#1$}}{%
    $\scriptscriptstyle#2$}}}

\newcommand{\mydprime}{\prime\prime}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  2.b.logic and set theory     %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\Exists}{\exists}
\DeclareMathOperator{\Forall}{\forall}
\newcommand{\Logiceq}{\Longleftrightarrow}
\newcommand{\logiceq}{\Leftrightarrow}
\newcommand{\logicand}{\; \&\& \;}
\newcommand{\Tiff}{{\itshape iff}}
\newcommand{\sucht}{\,{}:\,}
\newcommand{\cond}{\; | \;}
\newcommand{\setcond}[2]{\ifthenelse{\isempty{#2}}{\{#1\}}{\{#1\cond{}#2\}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  2.c.topological and metric space  %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\interior}[1]{\mathrm{int}\,{}#1}
\newcommand{\clos}[1]{#1^{-}}
\newcommand{\bound}[1]{\partial #1}
\newcommand{\diam}[1]{\mathrm{diam}\,{}#1}
\newcommand{\supm}[1]{\mathrm{sup}\,{}#1}
\newcommand{\infm}[1]{\mathrm{inf}\,{}#1}
\newcommand{\homot}{\simeq}
\newcommand{\pathhmt}{\sim}
\newcommand{\pathprod}{\cdot}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  2.d.matrix  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \newcommand{\tr}{\mathrm{Tr}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 3.physics-related %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% 3.a. general physics  %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{physics}
    %CCC braket command is more user friendly in this package than in the \usepckage{braket} with automatic sizing
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% 3.b.general high energy physics  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{braket}
\usepackage{cancel}
    %CCC This package provide \cancel{} to draw crossline in its argument. I think that \cancel is better to look than \slashed
    \def\slashed#1{\cancel{#1}}
        %CCC this is for compatibility purpose

\newcommand{\norord}[1]{\mathbf{:}\mathbin{#1}\mathbf{:}}
\newcommand{\Tord}[1]{T\left(#1\right)}
\newcommand{\gev}[1]{{#1\,\mathrm{GeV}}}
\newcommand{\gevSq}[1]{{#1\,\mathrm{GeV}^2}}
\newcommand{\mev}[1]{{#1\,\mathrm{MeV}}}
\newcommand{\mevSq}[1]{{#1\,\mathrm{MeV}^2}}


\newcommand{\FUU}{F_{UU}}
\newcommand{\FUUphi}{F_{UU}^{\cos\phi}}
\newcommand{\FUUIIphi}{F_{UU}^{\cos2\phi}}
\newcommand{\AUThminusS}{A_{UT}^{\sin\left(\phi_h-\phi_S\right)}}
\newcommand{\AUTIIIhminusS}{A_{UT}^{\sin\left(3\phi_h-\phi_S\right)}}
\newcommand{\AUThplusS}{A_{UT}^{\sin\left(\phi_h+\phi_S\right)}}
\newcommand{\ALThS}{A_{LT}^{\cos\left(\phi_h-\phi_S\right)}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  3.c.BLFQ  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\LCm}{{-}} 
\newcommand{\LCp}{{+}}
\newcommand{\LCpm}{{\pm}}
\newcommand{\LCmp}{{\mp}}
\newcommand{\LCperp}{{\perp}}
\newcommand{\LCperpinner}[2]{#1^{\perp} #2^{\perp}}
\newcommand{\LCinner}[2]{\frac{1}{2}#1^{+} \cdot #2^{-}+\frac{1}{2}#1^{-} \cdot #2^{+}-#1^{\perp} \cdot #2^{\perp}}

\newcommand{\nmax}{N_{\mathrm{max}}}
\newcommand{\perpSq}[1]{(#1^{\perp})^2}
\newcommand{\perpAbs}[1]{|#1^{\perp}|}
\let\ppSq\perpSq
\let\ppAbs\perpAbs

\newcommand{\fI}[1]{f_1^{#1}}
\newcommand{\fITperp}[1]{f_{1T}^{\perp #1}}
\newcommand{\gI}[1]{g_{1}^{#1}}
\newcommand{\gIL}[1]{g_{1L}^{#1}}
\newcommand{\gIT}[1]{g_{1T}^{#1}}
\newcommand{\hI}[1]{h_{1}^{#1}}
\newcommand{\hIT}[1]{h_{1T}^{#1}}
\newcommand{\hITperp}[1]{h_{1T}^{\perp #1}}
\newcommand{\hILperp}[1]{h_{1L}^{\perp #1}}
\newcommand{\hIperp}[1]{h_1^{\perp #1}}
\newcommand{\DI}[1]{D_1^{#1}}
\newcommand{\DITperp}[1]{D_{T}^{\perp #1}}
\newcommand{\HIperp}[1]{H_1^{\perp #1}}

\let\fITp\fITperp
\let\hIp\hIperp
\let\hILp\hILperp
\let\hITp\hITperp

\newcommand{\phiGM}[1]{\Phi_{#1}^{[\Gamma]}}
\newcommand{\phiLGM}{\Phi^{[\Gamma]}_{\Lambda^{\prime}\Lambda}}
\newcommand{\phiSGM}{\Phi^{[\Gamma]}(S)}
\newcommand{\phiAGGM}{\Phi^{[\Gamma]}(\theta,\varphi)}

\newcommand{\phip}[1]{\Phi_{#1}^{[\gamma^{+}]}}
\newcommand{\phiLp}{\Phi^{[\gamma^{+}]}_{\Lambda^{\prime}\Lambda}}
\newcommand{\phiSp}{\Phi^{[\gamma^{+}]}(S)}
\newcommand{\phiAGp}{\Phi^{[\gamma^{+}]}(\theta,\varphi)}

\newcommand{\phipV}[1]{\Phi_{#1}^{[\gamma^{+}\gamma^{5}]}}
\newcommand{\phiLpV}{\Phi^{[\gamma^{+}\gamma^{5}]}_{\Lambda^{\prime}\Lambda}}
\newcommand{\phiSpV}{\Phi^{[\gamma^{+}\gamma^{5}]}(S)}
\newcommand{\phiAGpV}{\Phi^{[\gamma^{+}\gamma^{5}]}(\theta,\varphi)}

\newcommand{\phijV}[2]{\Phi_{#2}^{[i\sigma^{#1}\gamma^{5}]}}
\newcommand{\phiLjV}[1]{\Phi^{[i\sigma^{#1}\gamma^{5}]}_{\Lambda^{\prime}\Lambda}}
\newcommand{\phiSjV}[1]{\Phi^{[i\sigma^{#1}\gamma^{5}]}(S)}
\newcommand{\phiAGjV}[1]{\Phi^{[i\sigma^{#1}\gamma^{5}]}(\theta,\varphi)}


